Adaptive Patching for High-resolution Image Segmentation with Transformers

Attention-based models are proliferating in the space of image analytics, including segmentation. The standard method of feeding images to transformer encoders is to divide the images into patches and then feed the patches to the model as a linear sequence of tokens. For high-resolution images, e.g. microscopic pathology images, the quadratic compute and memory cost prohibits the use of an attention-based model, if we are to use smaller patch sizes that are favorable in segmentation. The solution is to either use custom complex multi-resolution models or approximate attention schemes. We take inspiration from Adapative Mesh Refinement (AMR) methods in HPC by adaptively patching the images, as a pre-processing step, based on the image details to reduce the number of patches being fed to the model, by orders of magnitude. This method has a negligible overhead, and works seamlessly with any attention-based model, i.e. it is a pre-processing step that can be adopted by any attention-based model without friction. We demonstrate superior segmentation quality over SoTA segmentation models for real-world pathology datasets while gaining a geomean speedup of $6.9\times$ for resolutions up to $64K^2$, on up to $2,048$ GPUs.

==> tables/aux.tex <==
\begin{table*}[t]
\caption{\edit{WAHIB: TO BE CHANGED BY MERGING WITH THE OTHER TABLE. DON't TOUCH} A summary for different long sequence training methods. \emph{Serial} methods may need to be used on top of parallelism schemes. \emph{$l_x$}= sequence length; \emph{N}= number of GPU workers; \emph{H}= number of hierarchical levels; \emph{Z}= number of non-zeros.}
\label{tab:related_work}
\resizebox{\linewidth}{!}{
\centering
\begin{tabular}{|c|l|l|l|l|l|l|l|l|l|} 
\hline
\textbf{Approach}                                                                       & \textbf{Method}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Accuracy}\\\textbf{~Loss}\end{tabular}}                                                                        %\textbf{Accuracy \\Loss}  
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Serial/}\\\textbf{~Distributed}\end{tabular}}
%& \textbf{Serial\textbackslash Distributed}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Memory}\\\textbf{~(per worker)}\end{tabular}} %\textbf{Memory \\(per Worker)}                                                                       
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Compute}\\\textbf{~(per worker)}\end{tabular}} %\textbf{Compute \\(per Worker)}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Memory}\\\textbf{Total}\end{tabular}} %\textbf{Memory \\(agg.)}                                                                       
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Compute}\\\textbf{Total}\end{tabular}} %\textbf{Compute \\(agg.)}
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Comm.}\\\textbf{freq. per layer}\end{tabular}}                                                                        
& \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Practical}\\\textbf{~bottleneck}\end{tabular}} %\textbf{Practical \\bottleneck}
\\
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{Hierarchical }\\\textbf{Training}\end{tabular}
&\begin{tabular}[c]{@{}l@{}}HIPT~\cite{Chen22}, CrossViT~\cite{chen2021crossvit}\\ Hier. Trans.\cite{si21}, MEGABYTE~\cite{yu2023megabyte}\end{tabular} &
    No       & 
    Serial  &
    O($l_x^2H$)                             & 
    O($l_x^3H$)                                    & 
    N/A                             & 
    N/A                                    & 
    N/A &
    \begin{tabular}[c]{@{}l@{}}Train multiple \\models \end{tabular}\\ 
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{Attention }\\\textbf{Approximation}\end{tabular}
%\textbf{Attention \\ Approximation}
    &\begin{tabular}[c]{@{}l@{}} Reformer~\cite{reformer20}, Routing Trans.~\cite{Roy21} \\ Sparse Trans.~\cite{sparse-transformer19}, Longformer~\cite{Beltagy2020Longformer}\end{tabular} &
    Yes       & 
    Serial  &
    O($Z$)                             & 
    O($Z^3$)                                    & 
    N/A                             & 
    N/A                                    & 
    N/A &
    Low sparsity\\ 
\hline
\begin{tabular}[c]{@{}c@{}}\textbf{Sequence }\\\textbf{Parallelism}\end{tabular}
%\textbf{Attention \\ Approximation}
    &\begin{tabular}[c]{@{}l@{}} Partial Seq. Parallel~\cite{Li21,li2023lightseq} \\ Nvidia Seq. Para.\cite{Korthikanti22}, LSS~\cite{wang2023ultralong}\end{tabular} &
    No       & 
    Serial  &
    O($Z$)                             & 
    O($Z^3$)                                    & 
    N/A                             & 
    N/A                                    & 
    N/A &
    Low sparsity\\ 
\hline

\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Sequence }\\\textbf{Parallelism}\end{tabular}} 
    & \begin{tabular}[c]{@{}l@{}}Straightforward Seq. Parallel\\ \cite{Li21,li2023lightseq}  \end{tabular} & 
    %& \begin{tabular}[c]{@{}l@{}}Positional \\Interpolation~\cite{katharopoulos2018not} \end{tabular}  & 
    %\multirow{2}{*}{Implicit Ranking}                   & 
    \multirow{4}{*}{No}       & 
    \begin{tabular}[c]{@{}l@{}}Distributed \\ (partial aggr.)  \end{tabular}  &
    O(${l_x^2} / {N}$)                             & 
    O(${l_x^3} / {N}$)                                    & 
    O($l_x^2$)                             & 
    O($l_x^3$)                                    & 
    $\approx N^2$ &
    \begin{tabular}[c]{@{}l@{}}Frequent \\ communication  \end{tabular}
    \\ 
\cline{2-2}\cline{4-10}
    & \begin{tabular}[c]{@{}l@{}}Nvidia Seq. Parallel\\ \cite{Korthikanti22}  \end{tabular}  & 
           & 
    \begin{tabular}[c]{@{}l@{}}Distributed \\ (serial attention)  \end{tabular}   &
    O($l_x^2$)                             & 
    O($l_x^3$)                                    & 
    O($l_x^2$)                             & 
    O($l_x^3$)                                    & 
    $8$ &
    \begin{tabular}[c]{@{}l@{}}Attention not \\ distributed \end{tabular} \\
\cline{2-2}\cline{4-10}
    & \textbf{LSS Transformer (ours)}& 
    & 
    \begin{tabular}[c]{@{}l@{}}Distributed \\ (fully) \end{tabular}    &
    O(${l_x^2} / {N}$)                             & 
    O(${l_x^3} / {N}$)                                    & 
    O($l_x^2$)                             & 
    O($l_x^3$)                                    & 
    $2$ &
    - \\
\hline
\end{tabular}
}
\end{table*}

\begin{table*}[t]
	\centering
	\footnotesize
	\setlength{\tabcolsep}{5pt}
 \caption{Merits and Demerits of the two directions, attention matrix, linear attention and APF patches.}
 \resizebox{\linewidth}{!}{
	\begin{tabular}{c||c|c|c}
		\toprule [1.3pt]	
		\hline
		\multicolumn{1}{c||}{\textbf{Approach}} & \multicolumn{1}{c|}{\textbf{Method}} & \multicolumn{1}{c|}{\textbf{Merits \& Demerits} } & \multicolumn{1}{c}{\textbf{Time Complexity} } \\ 

		\hline
		\multirow{20}{*}{Attention Approx.}   
		&  Longformer~\cite{beltagy2020longformer}, ETC~\cite{ainslie2020etc}    & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} Better time complexity vs Transformer. \\
                \textbf{(-)} No sparse info.
            \end{tabular}& { $O(n\sqrt{n})$} \\
           
            \cline{2-4}
            &  {ETC \cite{ainslie2020etc}} & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} Better time complexity. \\
                \textbf{(-)} Relative position embedding requested.
            \end{tabular}& { $O(n\sqrt{n})$} \\
            \cline{2-4}
		&   {BigBird \cite{zaheer2020big} } & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} Theoretically proved time complexity.\\
                \textbf{(-)} High-order derivatives
            \end{tabular}& { $O(n\log{n})$} \\
		\cline{2-4}
            &  {Reformer \cite{kitaev2020reformer}} & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} Better time complexity. \\
                \textbf{(-)} Constrains on the keys that cannot be used for decoding tasks.
            \end{tabular}& { $O(n\log{n})$} \\
            \cline{2-4}
            &  {Sparse Attention \cite{child2019generating}}  & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} Introduced sparse factorizations of the attention. \\
                \textbf{(-)} Higher Time complexity.
            \end{tabular}& { $O(n\sqrt{n})$} \\
            & {Linear transformers \cite{katharopoulos2020transformers}}  & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} Introduced decomposition on softmax function. \\
                \textbf{(-)} Inferior results than standard transformers.
            \end{tabular}& { $O(n)$} \\
            \cline{2-4}
		& {Linformer \cite{katharopoulos2020transformers}}  & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} Fast adaptation \\
                \textbf{(-)} Assumption that self-attention is low rank.
            \end{tabular}& { $O(n)$} \\
            \cline{2-4}
		&  {Performer \cite{choromanski2020rethinking}} & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} No any priors such as sparsity or low-rankness \\
                \textbf{(-)} High-order derivatives
            \end{tabular}& { $O(n)$} \\
            \cline{2-4}
            &  {MH-IFT \cite{lorraine2020optimizing}} & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} Fast adaptation \\
                \textbf{(-)} High-order derivatives
            \end{tabular}& { $O(n)$} \\
            \hline
		\multirow{8}{*}{Linear attention} 
		& {Linear transformers \cite{katharopoulos2020transformers}}  & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} Introduced decomposition on softmax function. \\
                \textbf{(-)} Inferior results than standard transformers.
            \end{tabular}& { $O(n)$} \\
            \cline{2-4}
		& {Linformer \cite{katharopoulos2020transformers}}  & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} Fast adaptation \\
                \textbf{(-)} Assumption that self-attention is low rank.
            \end{tabular}& { $O(n)$} \\
            \cline{2-4}
		&  {Performer \cite{choromanski2020rethinking}} & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} No any priors such as sparsity or low-rankness \\
                \textbf{(-)} High-order derivatives
            \end{tabular}& { $O(n)$} \\
            \cline{2-4}
            &  {MH-IFT \cite{lorraine2020optimizing}} & \begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} Fast adaptation \\
                \textbf{(-)} High-order derivatives
            \end{tabular}& { $O(n)$} \\
		\hline
		\multirow{2}{*}{Ours} 
		&  {Adaptive Patching}          &\begin{tabular}[c]{@{}p{4cm}@{}}
                \textbf{(+)} No need for extra revising for the attention mechanism.   \\
                \textbf{(+)} Largely reduced computation cost while maintaining performance. \\
                \textbf{(-)} Reduction depends on the task feature of images. \\
            \end{tabular}& { $O(log^2n)$} \\
		\hline
		\bottomrule[1.3pt]
	\end{tabular}}
	\label{tab:linear_ref}
\end{table*}
